On Model and Data Scaling for Skeleton-based Self-Supervised Gait Recognition

Gait recognition from video streams is a challenging problem in computer vision biometrics due to the subtle differences between gaits and numerous confounding factors. Recent advancements in self-supervised pretraining have led to the development of robust gait recognition models that are invariant to walking covariates. While neural scaling laws have transformed model development in other domains by linking performance to data, model size, and compute, their applicability to gait remains unexplored. In this work, we conduct the first empirical study scaling on skeleton-based self-supervised gait recognition to quantify the effect of data quantity, model size and compute on downstream gait recognition performance. We pretrain multiple variants of GaitPT - a transformer-based architecture - on a dataset of 2.7 million walking sequences collected in the wild. We evaluate zero-shot performance across four benchmark datasets to derive scaling laws for data, model size, and compute. Our findings demonstrate predictable power-law improvements in performance with increased scale and confirm that data and compute scaling significantly influence downstream accuracy. We further isolate architectural contributions by comparing GaitPT with GaitFormer under controlled compute budgets. These results provide practical insights into resource allocation and performance estimation for real-world gait recognition systems.

==> tables/tab-compute-scaling-coeffs.tex <==
\begin{table}[hbt!]
    \centering
    \resizebox{0.45\textwidth}{!}{
        \begin{tabular}{llrr}
         &  & \multicolumn{2}{c}{$\alpha$} \\
         &  & Controlled & In-the-Wild \\
         & \% of Data &  &  \\
        \midrule
        \multirow[c]{7}{*}{$\mu = 1$} & 1.56 & 0.124 & 0.145 \\
         & 3.12 & 0.166 & 0.145 \\
         & 6.25 & 0.107 & 0.115 \\
         & 12.5 & 0.139 & 0.168 \\
         & 25.0 & 0.138 & 0.144 \\
         & 50.0 & 0.130 & 0.150 \\
         & 100.0 & 0.141 & 0.136 \\
        \cline{1-4}
        \multirow[c]{7}{*}{$\mu = 3$} & 1.56 & 0.092 & 0.138 \\
         & 3.12 & 0.149 & 0.138 \\
         & 6.25 & 0.173 & 0.154 \\
         & 12.5 & 0.153 & 0.184 \\
         & 25.0 & 0.164 & 0.171 \\
         & 50.0 & 0.194 & 0.169 \\
         & 100.0 & 0.177 & 0.176 \\
        \cline{1-4}
        \multirow[c]{7}{*}{$\mu = 5$} & 1.56 & 0.120 & 0.131 \\
         & 3.12 & 0.179 & 0.179 \\
         & 6.25 & 0.191 & 0.169 \\
         & 12.5 & 0.195 & 0.176 \\
         & 25.0 & 0.192 & 0.188 \\
         & 50.0 & 0.203 & 0.177 \\
         & 100.0 & 0.196 & 0.199 \\
        \cline{1-4}
        \end{tabular}}
        \hfill
    \resizebox{0.45\textwidth}{!}{
        \begin{tabular}{llrr}
         &  & \multicolumn{2}{c}{$\alpha$} \\
         & & Controlled & In-the-Wild \\
        & \% of Data &  &  \\
        \midrule
        \multirow[c]{7}{*}{$\mu = 2$} & 1.56 & 0.078 & 0.149 \\
         & 3.12 & 0.139 & 0.172 \\
         & 6.25 & 0.131 & 0.140 \\
         & 12.5 & 0.130 & 0.165 \\
         & 25.0 & 0.160 & 0.163 \\
         & 50.0 & 0.177 & 0.166 \\
         & 100.0 & 0.162 & 0.156 \\
        \cline{1-4}
        \multirow[c]{7}{*}{$\mu = 4$} & 1.56 & 0.110 & 0.115 \\
         & 3.12 & 0.136 & 0.151 \\
         & 6.25 & 0.185 & 0.155 \\
         & 12.5 & 0.181 & 0.172 \\
         & 25.0 & 0.189 & 0.161 \\
         & 50.0 & 0.192 & 0.186 \\
         & 100.0 & 0.182 & 0.167 \\
        \cline{1-4}
        \end{tabular}
}
    \caption{Caption - pentru gflops, ne da scaling bazat pe bugetul de antrenare {\color{red} TODO poate scoatem, sunt mai importante alea de mai jos cu trendul?}}
    \label{tab:data-scaling-coeffs}
\end{table}

==> tables/tab-gaitpt-gaitformer-sizes.tex <==
\begin{table}[hbt!]
    \centering
    \caption{Architectural details of the shallow and wide GaitPTv2 and the corresponding GaitFormer configuration. We show size configurations for both the spatial and temporal transformer layers at each of the four GaitPT stages. GFLOPs are computed for a forward pass with batch size of 1.}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{l|cccr|rr}
            \textbf{Model Name} & \textbf{Depth} & \textbf{d$_{model}$} & \textbf{n\_heads} & \textbf{Output Emb.} & \textbf{\# Params} & \textbf{\# GFLOPs} \\
            \midrule
            GaitPTv2-1 & \{2, 2, 4, 1\} & \{16, 64, 64, 128\} & \{1, 4, 4, 8\} & 64 & 1,194,144 & 0.246 \\
            GaitPTv2-2 & \{2, 2, 4, 1\} & \{32, 128, 128, 256\} & \{2, 8, 8, 16\} & 128 & 4,754,208 & 0.982 \\
            GaitPTv2-3 & \{2, 2, 4, 1\} & \{48, 192, 192, 384\} & \{3, 12, 12, 24\} & 192 & 10,680,736 & 2.210 \\
            GaitPTv2-4 & \{2, 2, 4, 1\} & \{64, 256, 256, 512\} & \{4, 16, 16, 32\} & 256 & 18,973,728 & 3.929 \\
            GaitPTv2-5 & \{2, 2, 4, 1\} & \{80, 320, 320, 640\} & \{5, 20, 20, 40\} & 320 & 29,633,184 & 6.138 \\
            GaitPTv2-6 & \{2, 2, 4, 1\} & \{96, 384, 384, 768\} & \{6, 24, 24, 48\} & 384 & 42,659,104 & 8.839 \\
            GaitPTv2-7 & \{2, 2, 4, 1\} & \{112, 448, 448, 896\} & \{7, 28, 28, 56\} & 448 & 58,051,488 & 12.03 \\
            \midrule
            GaitFormer-1 & 9 & 64 & 4 & 64 & 605,008 & 0.039 \\
            GaitFormer-2 & 9 & 128 & 8 & 128 & 2,402,688 & 0.156 \\
            GaitFormer-3 & 9 & 192 & 12 & 192 & 5,393,328 & 0.351 \\
            GaitFormer-4 & 9 & 256 & 16 & 256 & 9,576,928 & 0.624 \\
            GaitFormer-5 & 9 & 320 & 20 & 320 & 14,953,488 & 0.974 \\
            GaitFormer-6 & 9 & 384 & 24 & 384 & 21,523,008 & 1.403 \\
            GaitFormer-7 & 9 & 448 & 28 & 448 & 29,285,488 & 1.909 \\
            \end{tabular}
    }
    \label{tab:gaitpt-gaitformer-sizes}
\end{table}

